Opening Articulated Structures in the Real World

What does it take to build mobile manipulation systems that can competently operate on previously unseen objects in previously unseen environments? This work answers this question using opening of articulated structures as a mobile manipulation testbed. Specifically, our focus is on the end-to-end performance on this task without any privileged information, i.e. the robot starts at a location with the novel target articulated object in view, and has to approach the object and successfully open it. We first develop a system for this task, and then conduct 100+ end-to-end system tests across 13 real world test sites. Our large-scale study reveals a number of surprising findings: a) modular systems outperform end-to-end learned systems for this task, even when the end-to-end learned systems are trained on 1000+ demonstrations, b) perception, and not precise end-effector control, is the primary bottleneck to task success, and c) state-of-the-art articulation parameter estimation models developed in isolation struggle when faced with robot-centric viewpoints. Overall, our findings highlight the limitations of developing components of the pipeline in isolation and underscore the need for system-level research, providing a pragmatic roadmap for building generalizable mobile manipulation systems. Videos, code, and models are available on the project website: https://arjung128.github.io/opening-articulated-structures/

==> intended_demo.tex <==
\section{Intended Demonstration}
\seclabel{intended_demo}

We plan to conduct a live demonstration of our robotic system at the conference venue, ideally in a real, previously unseen kitchen or office-like environment. If that is not feasible, we will make use of novel isolated articulated objects for the demo. The demonstration will highlight the system's ability to autonomously open cabinets, drawers, and ovens it has never seen before, emphasizing its generalizability across diverse objects and environments. 
The project webpage can be found at \href{https://mosart-system.github.io/webpage}{mosart-system.github.io/webpage}, which includes roll-outs of \system on in-the-wild articulated objects, as well as the complete code of the system (also available at \href{https://github.com/mosart-system/code}{github.com/mosart-system/code}).



==> intro-v2.tex <==
\section{Introduction}
\seclabel{intro}



This paper develops and evaluates a system for pulling open
articulated objects (\eg drawers with prismatic joints,
cupboards with vertical hinges and ovens with horizontal hinges) in diverse
previously unseen real world environments (\figref{teaser}).
Opening such articulated objects presents hard technical challenges spanning
perception, planning, and last centimeter control. These include accurate
perception of object handles that are typically small and shiny, whole-body
planning to drive the end-effector along the task constraint (\ie trajectory
dictated by the articulating handle), and dealing with execution errors in a
task with low tolerances. All of these pieces have been studied at length in
isolation \cite{berenson2011task, sun2023opdmulti, karayiannidis2016adaptive}.
Yet, how these modules interact with one another and what matters for
successfully completing the task are not well understood. End-to-end learning
via imitation or reinforcement circumvents these issues but is itself difficult
because of the sample complexity of learning and the unavailability of
large-scale datasets for learning~\cite{gupta2023predicting}. 

In this paper, we take a modular approach (shown in
\figref{pipeline}) and bring to bear state-of-the-art modules for perception
and planning with a specific focus on studying how the different modules play
with one another. 
Specifically, for perception we extend a Mask RCNN model~\cite{he2017mask} to
also output articulation parameters. For planning, we extend
SeqIK~\cite{gupta2023predicting}, a trajectory optimization framework, to
produce whole body motion plans. 
Contrary to our expectation, just putting these two modules
together did not lead to a successful system because of last centimeter errors
in execution. Even slight inaccuracies in navigation and extrinsic camera
calibration cause the end-effector to just be slightly off from the handle
preventing grasping. To tackle this problem, we close the loop with
proprioceptive feedback: predictions from visual sensors get the end-effector
in the vicinity of the handle and the actual grasping is done by leveraging
contact sensors in the gripper and the arm.  The resulting MOdular System for opening ARTiculated objects (\system), achieves a 61\%
success rate at opening \textit{novel} drawers and cupboards in \textit{novel} environments.  It
also substantially outperforms end-to-end systems. While \system was developed
on drawers and cupboards, it easily extends to opening horizontal-hinged
toaster ovens and obtains a 80\% success rate.

Two other unique aspects of our study are a) the use of a {\it commodity mobile
manipulator} and b) extensive testing in previously unseen diverse real world
environments. Many previous papers have demonstrated specialized systems for
similar problems~\cite{jain2010pulling}. 
Constructing specialized hardware for a given task can simplify the task at
hand, at the cost of generality to other tasks.
Therefore, we test our proposed system using the Stretch RE2, a \textit{general
purpose} commodity mobile manipulator, \textit{without any hardware
modifications}.  Furthermore, this testing is conducted across 31 different
articulated objects in 10 different buildings. Testing sites include offices,
classrooms, apartments, office kitchenettes, and lounges as shown
in~\figref{teaser}. To the best of our knowledge, such extensive testing in
novel and diverse real world environments has never been done before. 





Our broad study sheds light on several questions about deploying such a system in the real world:
a) how does modular learning compare to end-to-end imitation learning,
b) what are the current bottlenecks in articulating objects in novel environments,  
c) how accurate should motion plans be for articulating objects, and 
d) what aspects of the system could benefit from machine learning?
Our large-scale experimental study reveals that our learned modular system 
outperforms end-to-end imitation learning methods (\secref{comparisons}). 
While it is possible that imitation learning may perform better with more data, 
scaling up such data collection remains a major challenge.
We find that perception is a major bottleneck for our current system, 
where inability to detect objects and handles accounts for 59\% of the
failures of the system (\figref{failures}, \secref{failure_mode_analysis}). 
This calls for broad datasets with labels for cabinet and drawer articulation 
parameters in \textit{diverse} environments.
Our study also reveals that control is surprisingly robust to mis-estimations in
the articulation parameters. Once the end-effector has acquired a firm grasp of
the handle, the system is able to sufficiently open the cabinet even
when the radius is off by $10cm$ (\secref{robustness} and \figref{robustness}).
Finally, errors in calibration and navigation compound to lead to failures
in grasping of the handle (\secref{failure_mode_analysis}). This motivates the need for a 
learned closed-loop visual last-centimeter handle grasping policy.




In summary, this paper presents the design and evaluation of a mobile
manipulation system to open novel articulated objects in novel environments
using a commodity mobile manipulator. Large scale testing across 13 test sites
in 10 buildings and 9 drawers, 22 cabinets and 3 toaster ovens
reveals guidance for practitioners building similar systems. 
Code is available in the supplementary material and will be 
made public for others to replicate and build upon.


==> intro-v3.tex <==
\section{Introduction (v3)}
\seclabel{intro}



This paper develops and evaluates a system for pulling open
articulated objects (\eg drawers with prismatic joints,
cupboards with vertical hinges and ovens with horizontal hinges) in diverse
previously unseen real world environments (\figref{teaser}).
Opening such articulated objects presents hard technical challenges spanning
perception, planning, and last centimeter control. These include accurate
perception of object handles that are typically small and shiny, whole-body
planning to drive the end-effector along the task constraint (\ie trajectory
dictated by the articulating handle), and dealing with execution errors in a
task with low tolerances. All of these pieces have been studied at length in
isolation \cite{berenson2011task, sun2023opdmulti, karayiannidis2016adaptive}.
Yet, how these modules interact with one another and what matters for
successfully completing the task are not well understood. End-to-end learning
via imitation or reinforcement circumvents these issues but is itself difficult
because of the sample complexity of learning and the unavailability of
large-scale datasets for learning~\cite{gupta2023predicting}. 

In this paper, we take a modular approach (shown in
\figref{pipeline}) and bring to bear state-of-the-art modules for perception
and planning with a specific focus on studying how the different modules play
with one another. 
Specifically, for perception we extend a Mask RCNN model~\cite{he2017mask} to
also output articulation parameters. For planning, we extend
SeqIK~\cite{gupta2023predicting}, a trajectory optimization framework, to
produce whole body motion plans. 
Contrary to our expectation, just putting these two modules
together did not lead to a successful system because of last centimeter errors
in execution. Even slight inaccuracies in navigation and extrinsic camera
calibration cause the end-effector to just be slightly off from the handle
preventing grasping. To tackle this problem, we close the loop with
proprioceptive feedback: predictions from visual sensors get the end-effector
in the vicinity of the handle and the actual grasping is done by leveraging
contact sensors in the gripper and the arm.  The resulting MOdular System for opening ARTiculated objects (\system), achieves a 61\%
success rate at opening \textit{novel} drawers and cupboards in \textit{novel} environments.  It
also substantially outperforms end-to-end systems. While \system was developed
on drawers and cupboards, it easily extends to opening horizontal-hinged
toaster ovens and obtains a 80\% success rate.

Two other unique aspects of our study are a) the use of a {\it commodity mobile
manipulator} and b) extensive testing in previously unseen diverse real world
environments. Many previous papers have demonstrated specialized systems for
similar problems~\cite{jain2010pulling}. 
Constructing specialized hardware for a given task can simplify the task at
hand, at the cost of generality to other tasks.
Therefore, we test our proposed system using the Stretch RE2, a \textit{general
purpose} commodity mobile manipulator, \textit{without any hardware
modifications}.  Furthermore, this testing is conducted across 31 different
articulated objects in 10 different buildings. Testing sites include offices,
classrooms, apartments, office kitchenettes, and lounges as shown
in~\figref{teaser}. To the best of our knowledge, such extensive testing in
novel and diverse real world environments has never been done before. 





Our broad study sheds light on several questions about deploying such a system in the real world:
a) how does modular learning compare to end-to-end imitation learning,
b) what are the current bottlenecks in articulating objects in novel environments,  
c) how accurate should motion plans be for articulating objects, and 
d) what aspects of the system could benefit from machine learning?
Our large-scale experimental study reveals that our learned modular system 
outperforms end-to-end imitation learning methods (\secref{comparisons}). 
While it is possible that imitation learning may perform better with more data, 
scaling up such data collection remains a major challenge.
We find that perception is a major bottleneck for our current system, 
where inability to detect objects and handles accounts for 59\% of the
failures of the system (\figref{failures}, \secref{failure_mode_analysis}). 
This calls for broad datasets with labels for cabinet and drawer articulation 
parameters in \textit{diverse} environments.
Our study also reveals that control is surprisingly robust to mis-estimations in
the articulation parameters. Once the end-effector has acquired a firm grasp of
the handle, the system is able to sufficiently open the cabinet even
when the radius is off by $10cm$ (\secref{robustness} and \figref{robustness}).
Finally, errors in calibration and navigation compound to lead to failures
in grasping of the handle (\secref{failure_mode_analysis}). This motivates the need for a 
learned closed-loop visual last-centimeter handle grasping policy.




In summary, this paper presents the design and evaluation of a mobile
manipulation system to open novel articulated objects in novel environments
using a commodity mobile manipulator. Large scale testing across 13 test sites
in 10 buildings and 9 drawers, 22 cabinets and 3 toaster ovens
reveals guidance for practitioners building similar systems. 
Code is available in the supplementary material and will be 
made public for others to replicate and build upon.

\system strongly outperforms the recent imitation learning system from
\cite{etukuru2024robot} that is trained on 1500 real world demonstrations for
opening articulated objects. Modularity enables \system to easily extended to
new articulation types \eg horizontal-hinged toaster ovens. Decoupled
perception and control  

We summarize the strengths of \system:
\begin{itemize}
\item While \system was developed on drawers and cupboards, its modular design
allows us to easily extend it to opening horizontal-hinged toaster ovens and
obtains a 80\% success rate.
\item \system outperforms imitation learning methods that are trained on
markedly larger amounts of real world data.
\end{itemize}

To summarize, our contributions lie not just in the system or its modules, but
in the experimental study, our findings, and the overall capability
demonstrated, as we summarize below:

\begin{itemize}
\item {\bf Experimental Study}: In the rich history of research on opening
cabinets and drawers, a large-scale evaluation on the task of opening cabinets
and drawers in the real world in a zero-shot manner, has simply never been done
before. Past works mostly show one-off demos, conduct evaluation on objects in
isolation, only do small scale studies, or only test part of the pipeline.
Thus, we believe that our experimental study is novel.
\item {\bf Findings}: Our large-scale study and failure mode analysis has revealed various insights: 
\begin{itemize}
\item Perception and not the precise control of the end-effector (to follow the
handle as the object articulates) is what makes this problem hard, contrary to
what prior work focuses
on~\cite{gupta2023predicting,karayiannidis2016adaptive,chitta2010planning}.
Control is surprisingly robust to mis-estimations in the articulation
parameters. 
\item The specific ways in which the perception system fails may inform future
research. It is not as much a failure in estimating articulation parameters,
but the detection of target objects and estimation of the handle location in 3D
that are the bottlenecks. Specifically, cabinets with meshed surfaces don’t get
detected and keyholes get mistaken as handles. It may be important to collect
datasets or build simulation assets that represent such variety. Apriori one
may not have thought to include such cases.
\item Not only did our modular system \system outperform the competing
imitation learning method RUM~\cite{etukuru2024robot}, we found the modular system to be
advantageous in other ways.  For example, we found it easy to extend it to a
new articulation type (horizontal-hinged toaster ovens). In comparison, an
imitation learning system will need to recollect training data for tackling a
new articulation type. Second, Detic-based perception module in \system 
continues to automatically improve as vision foundation models keep improving.
These takeaways are particularly useful in context of the
ongoing debate between modular learning and end-to-end learning. In fact,
recent works have adopted end-to-end learning to tackle the problem of opening
cabinets and drawers \cite{shafiullah2023bringing, xiong2024adaptive,
yang2023harmonic, gu2023maniskill2}. Thus, our paper provides useful
and relevant experimental evidence.
\end{itemize}
\item {\bf Overall Capability}: Finally, it may be surprising, but \system is
the first system that tackles the problem to as full an extent as we do
(zero-shot testing on novel objects in real environments with no privileged
information).  See discussion on other prior systems in \confirm{A11.4}.
Notable recent works on this problem \cite{shafiullah2023bringing,
xiong2024adaptive} require training on each test object using human-collected
demonstrations or an hour of robot-object interaction.
\end{itemize}


==> intro-v4.tex <==
\section{Introduction (v4)}
\seclabel{intro}

What does it take to enable a commodity mobile manipulator to successfully open
novel everyday articulated objects (\eg drawers, cabinets, ovens, \etc) in
diverse unseen real-world environments (\figref{teaser})?  Opening such
articulated objects presents hard technical challenges spanning perception,
planning, and last centimeter control. These include accurate perception of
object handles that are typically small and shiny, whole-body planning to drive
the end-effector along the task constraint (\ie trajectory dictated by the
articulating handle), and dealing with execution errors in a task with low
tolerances. All of these pieces have been studied at length in isolation
\cite{berenson2011task, sun2023opdmulti, karayiannidis2016adaptive}.  Yet, how
these modules interact with one another and what matters for successfully
completing the task are not well understood. End-to-end learning via imitation
or reinforcement circumvents these issues and are increasingly becoming the
tool of choice for these problems~\cite{etukuru2024robot, yang2023harmonic,
gu2023maniskill2}. In this work, we ask, a) as of today, how far can a modular
system that uses state-of-the-art modules go for this task? b) where does it
fail and what are the bottlenecks, c) how easy is it to improve its
performance or extend it? and most importantly d) {\it how does it 
fare against latest end-to-end learning methods?}

To enable this, we first put together a modular system (we will call it \system
for convenience) using Stretch RE 2 (a commodity mobile manipulator) for this
task using state-of-the-art methods. This includes a Mask RCNN
model~\cite{he2017mask} for inferring articulation parameters, a trajectory
optimization framework for producing whole body motion
plans~\cite{gupta2023predicting}, and some motion primitives for mitigating
the last centimeter errors. The system used some simulation assets for
training the perception model and a total of 1 drawer, 1 left-hinged cabinet,
and 1 right-hinged cabinet in the real world for all the development. We made
sure that we made no modifications to the robot, to retain its character as a
commodity mobile manipulator. 

Even though \system is the first system that tackles the problem to as full an
extent as we do (zero-shot testing on novel objects in real environments with
no privileged information, see discussion on other prior systems in
\confirm{A11.4}), \system is only moderately novel. Perhaps the only innovation
is in adapting each piece and putting them together. What is novel about our
paper are the experiments we did and the takeaways we found. We describe these
next.

We conducted large-scale tests to assess \system. This testing
was conducted across 31 different articulated objects in 10 different
buildings. Testing sites include offices, classrooms, apartments, office
kitchenettes, and lounges as shown in~\figref{teaser}. To the best of our
knowledge, such extensive testing in novel and diverse real world environments
has never been done before. \system obtained a 61\% success rate at this task.
The absolute success rate isn't very meaningful but the testing revealed many interesting failure modes that we discuss next.

Perhaps the most surprising finding was that, perception and not the precise
control of the end-effector (to follow the handle as the object articulates) is
what makes this problem hard, contrary to what prior work focuses
on~\cite{gupta2023predicting,karayiannidis2016adaptive,chitta2010planning}.
Inability to detect objects and handles accounts for 59\% of the failures of the
system (\figref{failures}, \secref{failure_mode_analysis}). Control was
surprisingly robust to mis-estimations in the articulation parameters. Once the
end-effector acquired a firm grasp of the handle, we found that the system
is able to sufficiently open the cabinet even when the radius is off by as much
as $10cm$ (\secref{robustness} and \figref{robustness}). 

Furthermore, the specific ways in which the perception system failed was also
revealing. It is not as much a failure in estimating articulation parameters,
but the detection of target objects and estimation of the handle location in 3D
are the bottlenecks. Specifically, cabinets with meshed surfaces don’t get
detected and keyholes get mistaken as handles. Future work should focus on
capturing data for such corner cases.


Beyond this testing, we also assessed \system from the point of view of
extensibility. Due to the modular design and use of foundation models for
perception, we found that \system could easily be extended to open other
articulation types such as objects with horizontal hinge joints (\eg ovens). We also
found it to work out of the box on a wide variety of handle types
(\secref{ovens_and_handles}).

To answer {\it how well does it compare to an end-to-end
learning system?}, we compare \system to the recent imitation learning work called RUM
from Etukuru \etal~\cite{etukuru2024robot}. RUM is trained on a large-scale dataset of
expert demonstrations: 1200 demos for opening cabinets, and 525 demonstrations
for opening drawers across approximately 40 environments, by far the largest
imitation learning dataset for this task. 
To our surprise, we find that the modular system, by far, outperforms this
latest end-to-end learning method. At the cost of dealing with errors of the up
stream modules, a modular system benefits from the additional data diversity
that can be absorbed by each individual module. This results is particularly
useful in context of the ongoing debate between modular learning and end-to-end
learning in robotics at large, and specifically for recent end-to-end learning
works that tackle the problem of opening cabinets and
drawers~\cite{shafiullah2023bringing, xiong2024adaptive, yang2023harmonic,
gu2023maniskill2}. 

To summarize, our unique first-of-its-kind study reveals the capabilities of
modular systems at opening articulated objects and sheds light on what are the
current bottlenecks. To facilitate further research and analysis, we have
open sourced the implementation of \system.





==> intro.tex <==
\section{Introduction}
\seclabel{intro}



This paper develops and evaluates a system for pulling open \textcolor{red}{articulated objects} in diverse previously unseen real world environments (Figure 1). %
\textcolor{red}{Articulated objects are ubiquitous in everyday environments and come in various forms: our focus is on the most common form of articulated objects, namely those with prismatic and hinge joints (e.g. drawers and cabinets).}
Opening articulated objects like cabinets and drawers presents hard technical challenges spanning perception, planning, and last centimeter control. These include accurate perception of object handles that are typically small and shiny, whole-body planning to drive the end-effector along the task constraint (\ie trajectory dictated by the articulating handle), and dealing with execution errors in a task with low tolerances. All of these pieces have been studied at length in isolation \cite{berenson2011task, sun2023opdmulti, karayiannidis2016adaptive}. Yet, how these modules interact with one another and what matters for successfully completing the task are not well understood. End-to-end learning via imitation or reinforcement circumvents these issues but is itself difficult because of the sample complexity of learning and the unavailability of large-scale datasets for learning~\cite{gupta2023predicting}. We take a modular approach (shown in \figref{pipeline}) and bring to bear state-of-the-art modules for perception and planning with a specific focus on studying how the different modules play with one another. 


Specifically, for perception we extend a Mask RCNN model~\cite{he2017mask} to also output articulation parameters. For planning, we extend SeqIK~\cite{gupta2023predicting}, a recently proposed trajectory optimization framework, to produce whole body motion plans. Contrary to our expectation, just putting these two modules together did not lead to a successful system because of last centimeter errors in execution. Even slight inaccuracies in navigation and extrinsic camera calibration cause the end-effector to just be slightly off from the handle preventing grasping. To tackle this problem, we close the loop with proprioceptive feedback: predictions from visual sensors gets the end-effector in the vicinity of the handle and the actual grasping is done by leveraging contact sensors in the gripper and the arm.

Two other unique aspects of our study are a) the use of a {\it commodity mobile manipulator} and b) extensive testing in previously unseen diverse real world environments. Many previous papers have demonstrated specialized systems for similar problems~\cite{jain2010pulling}. 
Constructing specialized hardware for a given task can simplify the task at hand, at the cost of generality to other tasks.
Therefore, we test our proposed system using the Stretch RE2, a \textit{general
purpose} commodity mobile manipulator, \textit{without any hardware modifications}. 
Furthermore, this testing is conducted across 31 different articulated objects in 10 different buildings. Testing sites include offices, classrooms, apartments, office kitchenettes, and lounges as shown in Figure 1.
Our system, \system ~\ags{broaden name?} achieves a 61\% zero-shot success rate across this challenging test bed.





Our broad study sheds light on several questions about deploying such a system in the real world:
a) how does modular learning compare to end-to-end imitation learning,
b) what are the current bottlenecks in articulating objects in novel environments,  
c) how accurate should motion plans be for articulating objects, 
\textcolor{red}{d) whether the system is general enough to work on other articulation types and diverse handles}, and
e) what aspects of the system could benefit from machine learning?
Our large-scale experimental study reveals that our learned modular system 
outperforms end-to-end imitation learning methods (\secref{comparisons}). 
While it is possible that imitation learning may perform better with more data, 
scaling up such data collection remains a major challenge.
We find that perception is a major bottleneck for our current system, 
where inability to detect objects and handles accounts for 59\% of the
failures of the system (\figref{failures}, \secref{failure_mode_analysis}). 
This calls for broad datasets with labels for cabinet and drawer articulation 
parameters in \textit{diverse} environments.
Our study also reveals that control is surprisingly robust to mis-estimations in
the articulation parameters. Once the end-effector has acquired a firm grasp of
the handle, the system is able to sufficiently open the cabinet even
when the radius is off by $10cm$ (\secref{robustness} and \figref{robustness}).
\textcolor{red}{Furthermore, we find that our modular approach can be easily extended to open other articulation types such as objects with horizontal hinge joints (e.g. ovens), and works on a wide variety of handle types (\secref{ovens_and_handles}).}
Finally, errors in calibration and navigation compound to lead to failures
in grasping of the handle (\secref{failure_mode_analysis}). This motivates the need for a 
learned closed-loop visual last-centimeter handle grasping policy.




In summary, this paper presents the design and evaluation of a mobile manipulation system to open cabinets and drawers using a commodity mobile manipulator. Large scale testing across 13 test sites in 10 buildings and 31 different cabinets and drawers reveals guidance for practitioners building similar systems. We will release code for others to replicate our results and build upon our system. 


==> rebuttal_modularity_v1.tex <==
\textbf{Modularity.} 
Yes, we agree that our modular design provides generalization within the constraints of the structure and may lack the capabilities to go beyond them.
However, we also demonstrate that an end-to-end learning approach trained on $1000+$ demonstrations [\textcolor{blue}{12}] struggles to generalize even for the one task it was trained on, and extending it to go beyond the learned capabilities would require collecting yet another large dataset, which may be infeasible for each and every task.
The ``bitter lesson" is an interesting point: unlike language and vision domains, where data is plentiful, robotics faces unique challenges that raise questions about whether we will ever achieve the data volume needed for end-to-end approaches to demonstrate true generalization, and if so, how long this will take.
Numerous attempts to scale up data for robotics \cite{zhao2024alohaunleashed}[\textcolor{blue}{12}] have demonstrated that even after many months of collecting data, learning a generalizable policy using end-to-end learning remains out of reach. 



Recent work in related robotics problems supports this view—from navigation systems \cite{gervet2022navigating} to other mobile manipulation systems on humanoids \cite{he2024omnih2o} and quadrupeds \cite{ha2024umilegs}, successful approaches have employed modular architectures rather than purely end-to-end learning. Furthermore, from a benchmarking perspective, our system provides a strong baseline for a challenging mobile manipulation task that current imitation learning approaches have yet to surpass. As an experimental field, we can measure rather than merely debate these tradeoffs, and the evidence suggests that while scaling data is certainly one promising avenue, it is neither the only approach nor guaranteed to be the long-run winner for robotics challenges.


==> rebuttal_modularity_v2.tex <==
\textbf{Modularity and the Bitter Lesson.} That's precisely a question that our work provides hard numbers for. \system is a modular system that outperforms RUM [\textcolor{blue}{12}], a state-of-the-art imitation learning (IL) system by an absolute 35\%. Note, this IL system was already \emph{scaled-up}: it used $1000+$ demos for training. 
With enough data end-to-end learning \textit{may} prevail, but unlike language and vision domains where data is plentiful, robotics faces unique challenges that raise questions about whether we will \textit{ever} achieve the data volume needed for true generalization (simulation could also provide scale but the sim-to-real gap remains a major hurdle).

Also, the bitter lesson may not always hold.
The success of NeRFs entirely relies on embedding volumetric rendering into learning. Perhaps, modularity is a similar structure to make robotic systems effective. There is increasing evidence pointing in this direction: \cite{gervet2022navigating} shows that a modular system outperforms a scaled-up IL/RL system for navigation, while \cite{he2024omnih2o} separates perception + high-level reasoning from low-level whole-body control for humanoid control. Furthermore, a modular system doesn't have to be anti-scaling. Rather, modularity can be very much pro-scaling: each individual module can be scaled up to absorb much more data than a monolithic end-to-end system. For example, the perception module in \system is trained on Internet images, far surpassing the data and diversity that an IL system would be exposed to.



As an experimental field, we can measure rather than merely debate these tradeoffs.
From a benchmarking perspective, \system provides a strong baseline for a challenging mobile manipulation task that current end-to-end learning approaches have yet to surpass.
While scaling data for end-to-end learning is one promising avenue, it is neither the only approach nor guaranteed to be the long-run winner for robotics. 
This was a very interesting point raised by the Area Chair, and we will include such a discussion in the revised version.


==> rebuttal_modularity_v3.tex <==














\textbf{Modularity and the Bitter Lesson.}
This is precisely a question that our work provides hard numbers for.
\system is a modular system that outperforms a state-of-the-art imitation learning (IL) system [\textcolor{blue}{12}] by an absolute 35\%, even when the IL system is trained on 1000+ real world demonstrations. 
While it seems likely that with enough data end-to-end learning may prevail, unlike language and vision domains where data is plentiful, robotics faces unique challenges that raise questions about whether we will ever achieve the data volume needed for end-to-end approaches to demonstrate true generalization.
While it seems that with enough data end-to-end learning \textit{may} prevail, unlike language and vision domains where data is plentiful, robotics faces unique challenges that raise questions about whether we will \textit{ever} achieve the data volume needed for end-to-end approaches to demonstrate true generalization.

Furthermore, recent work indicates that modularity and scaling are not mutually exclusive but rather complementary approaches that can amplify each other.
\cite{gervet2022navigating} shows that a modular system allows for scaling up certain modules to ultimately outperform a scaled-up end-to-end learning systems for navigation, while \cite{he2024omnih2o} separate perception + high-level reasoning from low-level whole-body control for humanoid control.
In this way, each individual module can be scaled up to absorb much more data than a monolithic end-to-end system. Similarly, the perception module in \system is trained on Internet images, far surpassing the data and diversity that an IL system would be exposed to.

As an experimental field, we can measure rather than merely debate these tradeoffs.
From a benchmarking perspective, \system provides a strong baseline for a challenging mobile manipulation task that current end-to-end learning approaches have yet to surpass.
While scaling data for end-to-end learning is one promising avenue, it is neither the only approach nor guaranteed to be the long-run winner for robotics. 
This was a very interesting point raised by the Meta Reviewer, and we will include such a discussion in the revised version.

